Better to Ask in English: Evaluation of Large Language Models on English, Low-resource and Cross-Lingual Settings

Large Language Models (LLMs) are trained on massive amounts of data, enabling their application across diverse domains and tasks. Despite their remarkable performance, most LLMs are developed and evaluated primarily in English. Recently, a few multi-lingual LLMs have emerged, but their performance in low-resource languages, especially the most spoken languages in South Asia, is less explored. To address this gap, in this study, we evaluate LLMs such as GPT-4, Llama 2, and Gemini to analyze their effectiveness in English compared to other low-resource languages from South Asia (e.g., Bangla, Hindi, and Urdu). Specifically, we utilized zero-shot prompting and five different prompt settings to extensively investigate the effectiveness of the LLMs in cross-lingual translated prompts. The findings of the study suggest that GPT-4 outperformed Llama 2 and Gemini in all five prompt settings and across all languages. Moreover, all three LLMs performed better for English language prompts than other low-resource language prompts. This study extensively investigates LLMs in low-resource language contexts to highlight the improvements required in LLMs and language-specific resources to develop more generally purposed NLP applications.

==> sections/llms.tex <==
% \section{Background of LLMs}
% \label{sec:llms-backgrounds}

% In this section, we discussed the LLMs that are evaluated by employing zero-shot learning in this study.
% %gpt4
% \paragraph{Generative Pre-trained Transformer - 4 (GPT-4) \cite{openai2023gpt}} 
% GPT-4 is one of the best-performing multimodal large language models (LLM) that can generate text from textual and visual input. GPT-4 was developed by OpenAI and was published in 2023. The model can handle more complex tasks such as exhibiting human-level performance on many professional and academic benchmarks, including the academic exams, and entrance exams. GPT-4 has extended GPT-3 and provides improved alignment and scalability. GPT-4 is multilingual and supports around 26 languages. The model has around a trillion trainable parameters, and a context length of 8, 192 and 32, 768 tokens. In our study, we employed a context window comprising 8,192 tokens, which cost approximately $\$30$ per one million tokens.

% %llma2
% \paragraph{Llama 2 \cite{touvron2023llama}}
% Llama 2 consists of three pre-trained and fine-tuned LLMs (e.g. \textit{Llama-2–7b, Llama-2–13b}, and \textit{Llama-2–70b}), released by Meta AI in 2023. It is one of the largest, best-performing, and open-source LLMs available for research and commercial use. The Llama 2 AI models exhibit proficiency across a range of natural language processing (NLP) tasks. The models were trained on two trillion parameters with a context length of $4,096$ tokens. Llama 2 was trained on $40$\% more publicly available training data compared to Llama 1, thus increasing the knowledge base and contextual understanding of Llama 2. Despite $90$\% of the training data being English, Llama 2 is capable of generating results across more than $50$ languages. Llama 2 base models serve as foundational pre-trained models intended for customization through fine-tuning for specific applications, while Llama 2 chat models are already optimized for dialogue purposes. In our study, we used \textit{Llama-2–70b-chat} through huggingface API\footnote{\url{https://huggingface.co/inference-api/}}. 


% %gemini
% \paragraph{Gemini \cite{team2023gemini}}
% Gemini is a family of LLMs developed by Google DeepMind. It has three different variations such as Ultra, Pro, and Nano and each specializes in specific tasks. Furthermore, Nano has two variations with 1.8B (Nano-1) and 3.25B (Nano-2) parameters. The parameter sizes of the Ultra and Pro models are unknown and not provided in the technical report of Gemini. The model has a context length of $32,768$ token and provides better results and understanding for long texts. Gemini is multimodal and can generalize, understand, and operate on different types of data including text, image, audio, and video. The multilingual capabilities of the Gemini models provide results across 38 languages, including Bangla, English, and Hindi, however, Urdu is not currently supported by Gemini. Gemini uses both heuristic rules and model-based classifiers-based safety settings to filter harmful content in the provided prompt and block responses for those contents. In this study, we used the Gemini Pro version from Gemini's Family of LLMs, which costs around $\$10$ per million tokens.


